User Feedback and Sample Weighting for Ill-Conditioned Hand-Eye Calibration

Hand-eye calibration is an important and extensively researched method for calibrating rigidly coupled sensors, solely based on estimates of their motion. Due to the geometric structure of this problem, at least two motion estimates with non-parallel rotation axes are required for a unique solution. If the majority of rotation axes are almost parallel, the resulting optimization problem is ill-conditioned. In this paper, we propose an approach to automatically weight the motion samples of such an ill-conditioned optimization problem for improving the conditioning. The sample weights are chosen in relation to the local density of all available rotation axes. Furthermore, we present an approach for estimating the sensitivity and conditioning of the cost function, separated into the translation and the rotation part. This information can be employed as user feedback when recording the calibration data to prevent ill-conditioning in advance. We evaluate and compare our approach on artificially augmented data from the KITTI odometry dataset.

==> plots/data/conditions_data.tex <==
\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}, only marks]
table {%
100 1.67307857090058
1000 5.61158091133795
2000 10.7525183377921
3000 16.1499219298502
4000 20.9065173954847
5000 25.5693270459851
6000 29.841193873234
7000 33.7592884860272
8000 36.6951328411769
9000 39.9702495800851
10000 42.7983866050125
};


==> plots/data/errors_density_rot.tex <==
\addplot [colormap/viridis, only marks, scatter, scatter src=explicit]
table [x=x, y=y, meta=colordata]{%
x  y  colordata
0.00272748477704898 0.00265525303554242 5.672631151835705
0.0185571893152676 0.0181601529983891 5.522346583631905
0.0407934333730956 0.0410838913396976 5.199178365279428
0.00206668798797773 0.00198415599501279 10.980448377345054
0.017407029579231 0.0171772059829613 10.432267762660512
0.0342039884797195 0.0363882903459686 9.204472434578186
0.00166667180675347 0.00152940844919536 16.64860449262726
0.0139139081920843 0.0134068649136007 15.458211569456202
0.0274196512587972 0.0294730220392522 12.833193080586852
0.00134507645940239 0.00122130980616141 21.73986486907905
0.011909210588817 0.0117637008515759 19.760065101472076
0.0225565500975576 0.0245427262287223 15.717239197372209
0.00125217128498137 0.00118582583240406 26.785234430618072
0.0137125570117641 0.013321563812693 23.897488139766672
0.0230121643487143 0.0240321519607317 18.286717892306797
0.00103273859332228 0.000984902352731835 31.48237360997383
0.0133251434732183 0.0128065504477819 27.60311143303598
0.019916998804494 0.0216632638636843 20.35149994686144
0.00109318379338298 0.0010133405911436 35.84822767791432
0.011733208750341 0.0113966831312094 30.927953981158492
0.0227160440090557 0.0265571193188633 22.02792768355833
0.00107275979469539 0.00100881075608239 39.16551206989893
0.0112776019803116 0.010933267055815 33.35225884590508
0.0216450335894319 0.025485756921536 23.13650420910812
0.00101474334444558 0.000955621336997481 42.93672862759807
0.0102775914675753 0.0100853430231015 35.96148256246386
0.020617307164158 0.0248990474252317 24.38856064076712
0.000926609171989009 0.00086781802448242 46.16070388339313
0.00967109935252898 0.00952041339203344 38.27021355499227
0.0208657271452701 0.0261647559149194 25.453766561905084
};

==> plots/data/errors_density_trans.tex <==
\addplot [colormap/viridis, only marks, scatter, scatter src=explicit]
table [x=x, y=y, meta=colordata]{%
x  y  colordata
1.09356647203578 1.07008173818948 5.672631151835705
13.07484255842 12.9419174567534 5.522346583631905
21.8638239001692 21.1915999148529 5.199178365279428
0.926911457288202 0.888511298846428 10.980448377345054
10.8077811676148 10.0966971491413 10.432267762660512
24.7673083715154 23.5087807689465 9.204472434578186
0.77024441520837 0.742253292259512 16.64860449262726
10.212550794525 8.62495918639518 15.458211569456202
19.746896455407 16.7442481390301 12.833193080586852
0.782291676975557 0.742548149489187 21.73986486907905
9.54136727256693 7.68068653210099 19.760065101472076
19.680553669273 15.9821650726708 15.717239197372209
0.730996151058853 0.701098376518671 26.785234430618072
8.5721794056154 7.00822710818453 23.897488139766672
17.0027914571666 15.8613211731519 18.286717892306797
0.70441424405414 0.686968218398122 31.48237360997383
9.38891922374051 7.01277046242774 27.60311143303598
13.5670531285857 12.6195281966643 20.35149994686144
0.696012336554951 0.691993859767796 35.84822767791432
10.2118490220586 7.17372470400852 30.927953981158492
16.6063652014268 11.6310148351814 22.02792768355833
0.649652180300521 0.658083766184872 39.16551206989893
10.3178137735338 7.00106953027203 33.35225884590508
15.2756533787296 11.2903352617876 23.13650420910812
0.632704214643617 0.647306547257952 42.93672862759807
9.79695688347535 6.66064712886482 35.96148256246386
17.438210459139 11.2743293544261 24.38856064076712
0.578230340156086 0.615940354694375 46.16070388339313
8.96334249092507 6.17685374886891 38.27021355499227
17.4338455857101 11.7195620223948 25.453766561905084
};

==> plots/data/errors_kmeans_rot.tex <==
\addplot [colormap/viridis, only marks, scatter, scatter src=explicit]
table [x=x, y=y, meta=colordata]{%
x  y  colordata
0.00272748477704898 0.00580761000862538 5.672631151835705
0.0185571893152676 0.0485902669478305 5.522346583631905
0.0407934333730956 0.131327280014027 5.199178365279428
0.00206668798797773 0.00301734544629166 10.980448377345054
0.017407029579231 0.0526365499538946 10.432267762660512
0.0342039884797195 0.117800974516952 9.204472434578186
0.00166667180675347 0.00483104224353638 16.64860449262726
0.0139139081920843 0.0549928130590031 15.458211569456202
0.0274196512587972 0.120503934585326 12.833193080586852
0.00134507645940239 0.00442398084430302 21.73986486907905
0.011909210588817 0.050899143361845 19.760065101472076
0.0225565500975576 0.118177370027898 15.717239197372209
0.00125217128498137 0.00263329431725658 26.785234430618072
0.0137125570117641 0.0443525905875716 23.897488139766672
0.0230121643487143 0.0631455204324407 18.286717892306797
0.00103273859332228 0.00409819682783152 31.48237360997383
0.0133251434732183 0.0527760805226081 27.60311143303598
0.019916998804494 0.0813330815322308 20.35149994686144
0.00109318379338298 0.00233373053220611 35.84822767791432
0.011733208750341 0.0393480041172806 30.927953981158492
0.0227160440090557 0.0867011924753776 22.02792768355833
0.00107275979469539 0.00232055659556215 39.16551206989893
0.0112776019803116 0.0438696304641449 33.35225884590508
0.0216450335894319 0.0849665058266137 23.13650420910812
0.00101474334444558 0.00286136640112306 42.93672862759807
0.0102775914675753 0.0376744642189512 35.96148256246386
0.020617307164158 0.0847632115122306 24.38856064076712
0.000926609171989009 0.00316391294754744 46.16070388339313
0.00967109935252898 0.0306393863193645 38.27021355499227
0.0208657271452701 0.0873841438061111 25.453766561905084
};

==> plots/data/errors_kmeans_trans.tex <==
\addplot [colormap/viridis, only marks, scatter, scatter src=explicit]
table [x=x, y=y, meta=colordata]{%
x  y  colordata
1.09356647203578 2.0828974693663 5.672631151835705
13.07484255842 20.8887764788489 5.522346583631905
21.8638239001692 62.2496187421671 5.199178365279428
0.926911457288202 1.74225876435204 10.980448377345054
10.8077811676148 23.8825654872788 10.432267762660512
24.7673083715154 72.994489402307 9.204472434578186
0.77024441520837 1.74899180958292 16.64860449262726
10.212550794525 23.1245733050915 15.458211569456202
19.746896455407 64.5153896412637 12.833193080586852
0.782291676975557 1.89797701524644 21.73986486907905
9.54136727256693 18.9220674669102 19.760065101472076
19.680553669273 51.9314409098672 15.717239197372209
0.730996151058853 1.66826320081271 26.785234430618072
8.5721794056154 22.0012878943892 23.897488139766672
17.0027914571666 43.5987845940061 18.286717892306797
0.70441424405414 1.66369431693839 31.48237360997383
9.38891922374051 18.7107356787706 27.60311143303598
13.5670531285857 53.69489996326 20.35149994686144
0.696012336554951 1.18829485933396 35.84822767791432
10.2118490220586 18.2499879589266 30.927953981158492
16.6063652014268 51.6933378657571 22.02792768355833
0.649652180300521 1.32116918525363 39.16551206989893
10.3178137735338 25.6537965278247 33.35225884590508
15.2756533787296 46.6172044820549 23.13650420910812
0.632704214643617 1.49446161605429 42.93672862759807
9.79695688347535 14.3016105915622 35.96148256246386
17.438210459139 51.1455613472415 24.38856064076712
0.578230340156086 1.43221082846662 46.16070388339313
8.96334249092507 17.3633127079068 38.27021355499227
17.4338455857101 39.6650743449581 25.453766561905084
};

==> plots/data/parameters_rot.tex <==
\addlegendimage{empty legend}
\addlegendentry{\hspace{-1.7em}\(\displaystyle n^{(\mathrm{uneven})}\)}

\addlegendimage{empty legend}
\addlegendentry{\hspace{-1.7em}(density)}

\addplot [very thick, steelblue31119180]
table {%
0.05 0.0235854686413083
0.1 0.02119550389164
0.15 0.0180589232009739
0.2 0.016146245098108
0.25 0.0153733150570526
};
\addlegendentry{\(\displaystyle 10^2\)}

\addplot [very thick, darkorange25512714]
table {%
	0.05 0.0120996343945789
	0.1 0.00999582740159056
	0.15 0.00909821973118875
	0.2 0.00868271795875194
	0.25 0.00855722575825152
};
\addlegendentry{\(\displaystyle 10^4\)}

\addplot [very thick, forestgreen4416044]
table {%
	0.05 0.00443625949765867
	0.1 0.00403623319380552
	0.15 0.00391775899989493
	0.2 0.00389952849562937
	0.25 0.00392273131162343
};
\addlegendentry{\(\displaystyle 10^5\)}


\addlegendimage{empty legend}
\addlegendentry{\hspace{-1.7em}(VQ)}

\addplot [very thick, steelblue31119180, densely dashed]
table {%
0.05 0.0413698029395637
0.1 0.0331272038118445
0.15 0.0364568231852034
0.2 0.0294955358431456
0.25 0.0306355410045804
};
\addlegendentry{\(\displaystyle 10^2\)}

\addplot [very thick, darkorange25512714, densely dashed]
table {%
0.05 0.0479841686291702
0.1 0.0329270574615341
0.15 0.0252827031328623
0.2 0.02842068656636
0.25 0.0334928858398049
};
\addlegendentry{\(\displaystyle 10^3\)}

\addplot [very thick, forestgreen4416044, densely dashed]
table {%
0.05 0.0330464095384452
0.1 0.0239547730976393
0.15 0.0210940452560324
0.2 0.023137189526231
0.25 0.014313080698794
};
\addlegendentry{\(\displaystyle 10^4\)}

==> plots/data/parameters_trans.tex <==
\addplot [very thick, steelblue31119180]
table {%
0.05 6.74445476053867
0.1 6.71739361071765
0.15 6.33715114588067
0.2 6.12295151054887
0.25 5.99736344557498
};
\addplot [very thick, steelblue31119180, densely dashed]
table {%
0.05 14.3839756533452
0.1 8.13951623018177
0.15 17.189841906657
0.2 8.89314873392762
0.25 11.9765766387707
};
\addplot [very thick, darkorange25512714]
table {%
0.05 4.984596376638
0.1 5.09008574361982
0.15 4.99760519701291
0.2 4.77944066004499
0.25 4.62669747337624
};
\addplot [very thick, darkorange25512714, densely dashed]
table {%
0.05 19.7754311560498
0.1 13.6768189653973
0.15 11.4848114294206
0.2 11.119547236917
0.25 10.2021359556914
};
\addplot [very thick, forestgreen4416044]
table {%
0.05 2.64452569942668
0.1 2.59863609847634
0.15 2.36548202723726
0.2 2.19122368029997
0.25 2.12340704911547
};
\addplot [very thick, forestgreen4416044, densely dashed]
table {%
0.05 15.414026451884
0.1 11.0185396583753
0.15 9.55970428535351
0.2 7.46464272191052
0.25 6.85427288426045
};


